Supervised ML Solution for Band Assignment in Dual-Band Systems with Omnidirectional and Directional Antennas

Many wireless networks, including 5G NR (New Radio) and future beyond 5G cellular systems, are expected to operate on multiple frequency bands. This paper considers the band assignment (BA) problem in dual-band systems, where the basestation (BS) chooses one of the two available frequency bands (centimeter-wave and millimeter-wave bands) to communicate with the user equipment (UE). While the millimeter-wave band might offer higher data rate, there is a significant probability of outage during which the communication should be carried on the (more reliable) centimeter-wave band. With mobility, the BA can be perceived as a sequential problem, where the BS uses previously observed information to predict the best band for a future time step. We formulate the BA as a binary classification problem and propose supervised Machine Learning (ML) solutions. We study the problem when both the BS and the UE use (i) omnidirectional antennas and (ii) both use directional antennas. In the omnidirectional case, we derive analytical benchmark solutions based on the Gaussian Process (GP) assumption for the inter-band shadow fading. In the directional case, where the labeling is shown to be complex, we propose an efficient labeling approach based on the Viterbi Algorithm (VA). We compare the performances for two channel models: (i) a stochastic channel and (ii) a ray-tracing based channel.

==> Features.tex <==

%
%\subsubsection{Features}\label{subsec:Fet}
%We consider six features, i.e., side information that are used as input to the learning solutions: ($\rm f_1$) the distance from the BS to the UE $d$ in meters, ($\rm f_2$) the angular position of the UE $\theta$ in rad, ($\rm f_3$) the received signal strength (or the SNR) in the cmWave band in dBm (or dB), ($\rm f_4$) similar quantities in the mmWave band,
%($\rm f_5$) the delay of the dominant MPC in seconds, and ($\rm f_6$) the AoD of the dominant MPC, where the dominant MPC is the one with the highest power. 

% The availability of the features depends on the system implementations. For instance, ($\rm f_1$) and ($\rm f_2$), i.e., $(d,\theta)$ (which represent the polar coordinates of the UE with respect to the BS), may be estimated using signal processing techniques or acquired by explicit feedback of the GPS data. To extract ($\rm f_5$) large bandwidth might be required, for ($\rm f_6$) the use of antenna arrays is necessary. Using both ($\rm f_3$) and ($\rm f_4$) is only reasonable for the sequential BA problem, but it may require additional effort or equipment at the UE side. We consider several combinations of the above features and discuss their effectiveness for BA.

%As typically done in ML, we perform pre-processing of the features, in particular we standardize the input features such that their mean is zero and the standard deviation is equal to one. In addition, we utilize the prior knowledge about the wireless propagation, for instance we use logarithmic scale for distances and power, as this may linearize their relation with one another.

==> Labeling.tex <==
\subsubsection{SISO}

\subsubsection{MIMO}

==> Tables/TblSeqRT.tex <==
\begin{table*}[!htb]
\vspace{0mm}
\centering
 \notsotiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\bf  Feat./Comb.  	  & \bf c-1   & \bf c-2   &\bf  c-3   &\bf c-4     & \bf c-5   & \bf c-6   	&\bf c-7 	& \bf c-8 	& \bf c-9 		& \bf c-10 	& \bf c-11  \\
\hline	
$\boldsymbol{d}$      &\checkmark &\checkmark &\checkmark  &           &           &			&           &           &           	&          	&           \\
\hline
$\boldsymbol{\theta}$ &\checkmark &\checkmark &\checkmark  &           &           &           	&           &           &           	&\checkmark &          \\
\hline
\bf cmWave            &           &\checkmark &\checkmark &\checkmark  &\checkmark &			&			&\checkmark & \checkmark	&\checkmark &\checkmark\\
\hline
\bf mmWave            &           &           & \checkmark &\checkmark &		   & \checkmark &		  	&           &  \checkmark	&          	&          \\
\hline
\bf Delay             &           &           &           &			   &           &           	&\checkmark &\checkmark &\checkmark		&          	& \checkmark\\
\hline
\bf AoD               &           &           &           &            &           &           	&\checkmark	&\checkmark &\checkmark		&			&          \\
%\hline  %\Xhline{2.3\arrayrulewidth} 
%\bf LSTM\textsubscript{opzd} $\boldsymbol{\bar{\mathcal{E}}_S}$   &.078/.115  &.066/.108  &.061/.102  &.07/.121    &.092/.16   &.096/.128   &.094/.13   &.073/.115  &.071/.124      &.072/.119	&.08/.132\\
%\bf LSTM\textsubscript{opzd} $\boldsymbol{\bar{\mathcal{L}}_S}$   &.048/.078  &.044/.074  &.041/.072    &.048/.085   &.061/.113  &.062/.089    &.065/.094  &.048/.08  &.046/.085      &.048/.085	&.054/.091\\
\hline 
\bf LSTM\textsubscript{bsk} $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.084/.114  &.068/.105  &.06/.103     &.07/.114   &.092/.147  &.082/.125    &.092/.138  &.067/.11  &.062/.106      &.072/.117	&.074/.125\\
\bf LSTM\textsubscript{bsk} $\boldsymbol{\bar{\mathcal{L}}_S}$	  &.051/.079  &.045/.075  &.041/.075     &.048/.082   &.061/.108  &.054/.089    &.063/.101  &.047/.077  &.042/.076      &.048/.082	&.049/.091\\
\hline 
\bf NN\textsubscript{H}	     $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.086/.11  &.083/.119  &.076/.116     &.107/.139   &.134/.162  &.12/.15    &.113/.147  &.098/.117  &.085/.117     &.099/.144	&.107/.152\\
\bf NN\textsubscript{H}	     $\boldsymbol{\bar{\mathcal{L}}_S}$   &.053/.073  &.052/.081  &.047/.078     &.068/.096   &.088/.114  &.078/.103    &.074/.105  &.063/.082  &.054/.081     &.063/.103	&.068/.106\\
%\hline 
%\bf GR 	      $\boldsymbol{\bar{\mathcal{E}}_S}$	    	      &.208/.211  &.138/.168  &.123/.156   &.125/.158   &.142/.17  &.125/.158    &.224/.224  &.138/.167  &.129/.156     &.137/.168	&.139/.169\\
%\bf GR 	      $\boldsymbol{\bar{\mathcal{L}}_S}$                  &.147/.15  &.093/.12  &.08/.109     &.082/.11   &.096/.121  &.082/.111    &.159/.16  &.092/.118  &.086/.109      &.092/.119	&.093/.12\\

\hline 
\bf GR\textsubscript{H}      $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.208/.211  &.134/.156  &.123/.15     &.125/.156   &.142/.17  &.122/.153    &.224/.231  &.138/.166  &.119/.155      &.137/.164	&.14/.168\\
\bf GR\textsubscript{H}       $\boldsymbol{\bar{\mathcal{L}}_S}$  &.149/.151  &.089/.11  &.08/.104     &.081/.108   &.096/.121  &.079/.106    &.16/.166  &.092/.117  &.078/.108      &.091/.116	&.093/.106\\

\hline 
\bf GP $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.183/.177 }  \\
\bf GP $\boldsymbol{\bar{\mathcal{L}}_S}$ 	 &\multicolumn{11}{|c|}{.127/.123 }  \\
\hline 
\bf GP\textsubscript{App}  $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.159/.174}  \\
\bf GP\textsubscript{App} $\boldsymbol{\bar{\mathcal{L}}_S}$ 	 &\multicolumn{11}{|c|}{.107/.119}  \\

\hline
\end{tabular}
\vspace{3mm}
\caption{Sequential BA: Performance of the learning techniques on ray-tracing data, under different feature availability, note that the percentage of points with labels equal to $"1"$ is approximately $30$\%.}
\vspace{-9mm}
\label{Tab:ResultsRay}
\vspace{-0mm}
\end{table*}

==> Tables/TblSeqRT_Antennas.tex <==
\begin{table*}[!htb]
\vspace{-3mm}
\centering
 \notsotiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\bf  Feat./Comb.  	  & \bf c-1   & \bf c-2   &\bf  c-3   &\bf c-4     & \bf c-5   & \bf c-6   	&\bf c-7 	& \bf c-8 	& \bf c-9 		& \bf c-10 	& \bf c-11  \\
\hline	
$\boldsymbol{d}$      &\checkmark &\checkmark &\checkmark  &           &           &			&           &           &           	&          	&           \\
\hline
$\boldsymbol{\theta}$ &\checkmark &\checkmark &\checkmark  &           &           &           	&           &           &           	&\checkmark &          \\
\hline
\bf cmWave            &           &\checkmark &\checkmark &\checkmark  &\checkmark &			&			&\checkmark & \checkmark	&\checkmark &\checkmark\\
\hline
\bf mmWave            &           &           & \checkmark &\checkmark &		   & \checkmark &		  	&           &  \checkmark	&          	&          \\
\hline
\bf Delay             &           &           &           &			   &           &           	&\checkmark &\checkmark &\checkmark		&          	& \checkmark\\
\hline
\bf AoD               &           &           &           &            &           &           	&\checkmark	&\checkmark &\checkmark		&			&          \\
\hline   
\multirow{4}{*}{LSTM}& 0.0771 & 0.0643 & 0.0619 & 0.0703 & 0.0939 & 0.0799 & 0.0957 & 0.0729 & 0.0646 & 0.0713 & 0.0793  \\ \cline{2-12}
    & 0.0801 & 0.0682 & 0.06 & 0.07 & 0.105 & 0.0829 & 0.1006 & 0.0704 & 0.0587 & 0.07 & 0.0806  \\ \cline{2-12}
    & 0.0808 & 0.068 & 0.0643 & 0.0713 & 0.0939 & 0.0802 & 0.0973 & 0.0698 & 0.0605 & 0.0691 & 0.0798  \\ \cline{2-12}
    & 0.0712 & 0.0582 & 0.053 & 0.0625 & 0.0957 & 0.0872 & 0.0858 & 0.0641 & 0.0596 & 0.0645 & 0.0728  \\ \cline{2-12}
\hline   \hline
\multirow{4}{*}{DNN}& .086 & .083 & .076 & .107 &.134 & .12 & .113 & .098 & .085 & .099 & .107  \\ \cline{2-12}
    & 0.0939 &0.0913 & 0.0857 & 0.1113 & 0.1356 & 0.1207 & 0.1449 & 0.0882 & 0.087 & 0.095 & 0.109  \\ \cline{2-12}
    & 0.092 & 0.089 & 0.084 & 0.108 & 0.1348 & 0.1206 & 0.1325 & 0.0895 & 0.082 & 0.1028 & 0.107  \\ \cline{2-12}
    & 0.082 & 0.093 & 0.077 & 0.1147 & 0.1309 & 0.119 & 0.136 & 0.089 & 0.0767 & 0.0949 & 0.1038  \\ \cline{2-12}
\hline   
%\multirow{4}{*}{GP}& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11  \\ \cline{2-12}
%    & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11  \\ \cline{2-12}
%    & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11  \\ \cline{2-12}
%    & 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 & 10 & 11  \\ \cline{2-12}
%\hline 

%\hline 
%\bf GP $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.183/.177 }  \\
%\bf GP $\boldsymbol{\bar{\mathcal{R}}_S}$ 	 &\multicolumn{11}{|c|}{.127/.123 }  \\
%\hline 
%\bf GP\textsubscript{App}  $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.159/.174}  \\
%\bf GP\textsubscript{App} $\boldsymbol{\bar{\mathcal{R}}_S}$ 	 &\multicolumn{11}{|c|}{.107/.119}  \\

\hline
\end{tabular}
\vspace{0mm}
\caption{Performance of the solutions on ray-tracing data under different feature availability. The percentage of points with labels equal to $"1"$ is approximately $30$\%. Results in rows 8-19 correspond to $U=4/U=8$.}
\vspace{-9mm}
\label{Tab:SeqResultsRT}
\vspace{-0mm}
\end{table*}

==> Tables/TblSeqRT_nr.tex <==
\begin{table*}[!htb]
\vspace{-3mm}
\centering
 \notsotiny
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\bf  Feat./Comb.  	  & \bf c-1   & \bf c-2   &\bf  c-3   &\bf c-4     & \bf c-5   & \bf c-6   	&\bf c-7 	& \bf c-8 	& \bf c-9 		& \bf c-10 	& \bf c-11  \\
\hline	
$\boldsymbol{d}$      &\checkmark &\checkmark &\checkmark  &           &           &			&           &           &           	&          	&           \\
\hline
$\boldsymbol{\theta}$ &\checkmark &\checkmark &\checkmark  &           &           &           	&           &           &           	&\checkmark &          \\
\hline
\bf cmWave            &           &\checkmark &\checkmark &\checkmark  &\checkmark &			&			&\checkmark & \checkmark	&\checkmark &\checkmark\\
\hline
\bf mmWave            &           &           & \checkmark &\checkmark &		   & \checkmark &		  	&           &  \checkmark	&          	&          \\
\hline
\bf Delay             &           &           &           &			   &           &           	&\checkmark &\checkmark &\checkmark		&          	& \checkmark\\
\hline
\bf AoD               &           &           &           &            &           &           	&\checkmark	&\checkmark &\checkmark		&			&          \\
%\hline  %\Xhline{2.3\arrayrulewidth} 
%\bf LSTM\textsubscript{opd} $\boldsymbol{\bar{\mathcal{E}}_S}$   &.078/.117  &.062/.103  &.062/.1  &.07/.12    &.094/.14   &.08/.132   &.098/.137   &.071/.114  &.061/.11      &.071/.12	&.081/.128\\
%\bf LSTM\textsubscript{opd} $\boldsymbol{\bar{\mathcal{R}}_S}$   &.048/.08  &.044/.074  &.041/.071    &.048/.085   &.061/.1  &.062/.092    &.065/.098  &.048/.08  &.046/.078      &.048/.086	&.054/.089\\
\hline 
\bf LSTM\textsubscript{std} $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.077/.117  &.064/.108  &.062/.1     &.07/.123   &.094/.14  &.08/.132    &.096/.134  &.073/.118  &.065/.111      &.071/.12	&.079/.126\\
%\bf LSTM\textsubscript{std} $\boldsymbol{\bar{\mathcal{R}}_S}$	  &.048/.081  &.044/.075  &.042/.071     &.048/.089   &.062/.1  &.053/.094    &.067/.096  &.049/.086  &.044/.08      &.047/.086	&.053/.09\\
\hline 
\bf NN\textsubscript{H}	     $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.086/.11  &.083/.119  &.076/.116     &.107/.139   &.134/.162  &.12/.15    &.113/.147  &.098/.117  &.085/.117     &.099/.144	&.107/.152\\
%\bf NN\textsubscript{H}	     $\boldsymbol{\bar{\mathcal{R}}_S}$   &.053/.073  &.052/.081  &.047/.078     &.068/.096   &.088/.114  &.078/.103    &.074/.105  &.063/.082  &.054/.081     &.063/.103	&.068/.106\\
%\hline 
%\bf GR 	      $\boldsymbol{\bar{\mathcal{E}}_S}$	    	      &.208/.211  &.138/.168  &.123/.156   &.125/.158   &.142/.17  &.125/.158    &.224/.224  &.138/.167  &.129/.156     &.137/.168	&.139/.169\\
%\bf GR 	      $\boldsymbol{\bar{\mathcal{L}}_S}$                  &.147/.15  &.093/.12  &.08/.109     &.082/.11   &.096/.121  &.082/.111    &.159/.16  &.092/.118  &.086/.109      &.092/.119	&.093/.12\\

\hline 
\bf GR\textsubscript{H}      $\boldsymbol{\bar{\mathcal{E}}_S}$	  &.208/.211  &.134/.156  &.123/.15     &.125/.156   &.142/.17  &.122/.153    &.224/.231  &.138/.166  &.119/.155      &.137/.164	&.14/.168\\
%\bf GR\textsubscript{H}       $\boldsymbol{\bar{\mathcal{R}}_S}$  &.149/.151  &.089/.11  &.08/.104     &.081/.108   &.096/.121  &.079/.106    &.16/.166  &.092/.117  &.078/.108      &.091/.116	&.093/.106\\

\hline 
\bf GP $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.183/.177 }  \\
%\bf GP $\boldsymbol{\bar{\mathcal{R}}_S}$ 	 &\multicolumn{11}{|c|}{.127/.123 }  \\
\hline 
\bf GP\textsubscript{App}  $\boldsymbol{\bar{\mathcal{E}}_S}$	 &\multicolumn{11}{|c|}{.159/.174}  \\
%\bf GP\textsubscript{App} $\boldsymbol{\bar{\mathcal{R}}_S}$ 	 &\multicolumn{11}{|c|}{.107/.119}  \\

\hline
\end{tabular}
\vspace{0mm}
\caption{Performance of the solutions on ray-tracing data under different feature availability. The percentage of points with labels equal to $"1"$ is approximately $30$\%. Results in rows 8-19 correspond to $U=4/U=8$.}
\vspace{-9mm}
\label{Tab:SeqResultsRT}
\vspace{-0mm}
\end{table*}

==> Tables/TblSeqStochNu1.tex <==
\begin{table*}[!htb]
\notsotiny
    \centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
\bf Feature / Combination                   		& {\bf c-1 } & \bf c-2   & \bf c-3   &\bf c-4    & \bf c-5    & \bf c-6   & \bf c-7    \\
\hline
 $\boldsymbol{d}$                           		&\checkmark  &\checkmark &           &\checkmark &\checkmark  &           &            \\
 \hline
 $\boldsymbol{\theta}$                      		&\checkmark  &           &\checkmark &\checkmark &\checkmark  &           &             \\
 \hline
\bf cmWave       Power                 		&            &\checkmark &\checkmark &\checkmark &\checkmark  &\checkmark & \checkmark \\
 \hline
\bf mmWave    Power                   		&            &           &           &           &\checkmark  &\checkmark &\\

 \hline \Xhline{2.4\arrayrulewidth}  
 %\bf LSTM\textsubscript{opd}  $\boldsymbol{\bar{\mathcal{E}}_S}$  	&  .178/.198 & .195/.214&.183/.238	 & .164/.196 &.159/.193	 &.192/.244	 &.206/.248   \\
 % \bf LSTM\textsubscript{opd}  $\boldsymbol{\bar{\mathcal{R}}_S}$  	&  .068/.077 & .081/.088	&.073/.1	 & .062/.078 &.062/.078	 &.077/.102	 &.083/.103   \\
 \hline 
  \bf  LSTM  $\boldsymbol{ \bar{\mathcal{E}}_S}$	&  .178/.198 & .193/.214	&.183/.233	 & .165/.192 &.163/.192	 &.191/.243	 &.206/.252   \\
%\bf  LSTM\textsubscript{std}  $\boldsymbol{\bar{\mathcal{R}}_S}$    &  .068/.077 & .078/.088	&.073/.099	 & .064/.076 &.065/.077	 &.079/.107	 &.083/.104   \\
 \hline 
 \bf NN\textsubscript{H}  $\boldsymbol{\bar{\mathcal{E}}_S}$  		&  .211/.216 & .216/.227&.197/.244	 & .192/.214 &.189/.207	 &.209/.251	 &.22/.257   \\
 % \bf   NN\textsubscript{H}  $\boldsymbol{\bar{\mathcal{R}}_S}$      	&  .08/.082 & .083/.087&.074/.101	 & .072/.082 &.071/.08	 &.081/.104	 &.085/.106 \\
 %\hline 
 %\bf GR $\boldsymbol{\bar{\mathcal{E}}_S}$  		&  .227/.242 & .22/.242  &.215/.252	 & .213/.241  &.207/.242	 &.214/.258	 &.221/.257   \\
 %    GR  $\boldsymbol{\bar{\mathcal{L}}_S}$ 	    &  .089/.099 & .085/.098&.083/.104	 & .082/.098 &.078/.099	 &.084/.107	 &.086/.106   \\
 \hline 
 \bf GR\textsubscript{H}  $\boldsymbol{\bar{\mathcal{E}}_S}$ 		&  .22/.225  & .22/.229	&.214/.25	 & .209/.225 &.198/.227	 &.211/.257	 &.221/.256   \\
%  \bf  GR\textsubscript{H}   $\boldsymbol{\bar{\mathcal{R}}_S}$ 		&  .085/.088 & .083/.089&.082/.103   & .079/.088 &.074/.088  &.081/.107	 &.086/.106   \\
 \hline  
 \bf GP   $\boldsymbol{\bar{\mathcal{E}}_S}$ &\multicolumn{7}{|c|}{.201/.226}  \\
%\bf	GP  $\boldsymbol{\bar{\mathcal{R}}_S}$ &\multicolumn{7}{|c|}{ .075/.088}  \\
  \hline 
   \bf GP\textsubscript{App}  $\boldsymbol{\bar{\mathcal{E}}_S}$ &\multicolumn{7}{|c|}{.221/.242}  \\
%   \bf GP\textsubscript{App} 	   $\boldsymbol{\bar{\mathcal{R}}_S}$ &\multicolumn{7}{|c|}{.082/.095}  \\
  \hline 
 \end{tabular}
 \vspace{-1mm}
  \caption{Sequential BA $\nu =1$: Performance of the learning over the stochastic data under different feature availability. Note that on average $47.9$\% of the labels are $"1"$. The first number in each entry in rows $6-17$ denotes the prediction error with $U=4$, and the second with $U=8$. }
   \vspace{-9mm}
 \label{Tab:ResultsSeqNu1}
\end{table*}
 

==> Tables/TblSeqStochNu19.tex <==
\begin{table*}[!htb]
\notsotiny
    \centering
 \begin{tabular}{|c|c|c|c|c|c|c|c|}
 \hline
\bf Feature / Combination                   		& {\bf c-1 } & \bf c-2   & \bf c-3   &\bf c-4    & \bf c-5    & \bf c-6   & \bf c-7    \\
\hline
 $\boldsymbol{d}$                           		&\checkmark  &\checkmark &           &\checkmark &\checkmark  &           &            \\
 \hline
 $\boldsymbol{\theta}$                      		&\checkmark  &           &\checkmark &\checkmark &\checkmark  &           &             \\
 \hline
\bf cmWave Power                            		&            &\checkmark &\checkmark &\checkmark &\checkmark  &\checkmark & \checkmark \\
 \hline
\bf mmWave Power                            		&            &           &           &           &\checkmark  &\checkmark &\\

 \hline \Xhline{2.4\arrayrulewidth}  
%\bf LSTM\textsubscript{opd} $\boldsymbol{\bar{\mathcal{E}}_S}$  	&  .166/.209 & .158/.204&.139/.203	 & .124/.184 &.103/.178	 &.119/.215	 &.166/.23   \\
%\bf LSTM\textsubscript{opzd} $\boldsymbol{\bar{\mathcal{R}}_S}$  	&  .068/.089 & .06/.084	&.052/.087	 & .046/.075 &.034/.074	 &.042/.096	 &.063/.097   \\
 \hline 
  \bf  LSTM\textsubscript{std} $\boldsymbol{\bar{\mathcal{E}}_S}$	&  .166/.204 & .158/.206	&.142/.203	 & .123/.185 &.107/.175	 &.119/.215	 &.166/.229   \\
%  \bf  LSTM\textsubscript{std} $\boldsymbol{\bar{\mathcal{R}}_S}$    &  .068/.085 & .062/.085	&.053/.087	 & .045/.077 &.037/.074	 &.042/.096	 &.063/.099   \\
 \hline 
 \bf NN\textsubscript{H} $\boldsymbol{\bar{\mathcal{E}}_S}$  		&  .196/.209 & .18/.211	&.155/.217	 & .147/.201 &.118/.195	 &.136/.231	 &.176/.233   \\
%   \bf   NN\textsubscript{H}  $\boldsymbol{\bar{\mathcal{R}}_S}$      	&  .077/.085 & .067/.084&.055/.091	 & .051/.081 &.036/.077	 &.042/.098	 &.066/.099 \\
 %\hline 
% \bf GR $\boldsymbol{\bar{\mathcal{E}}_S}$  		&  .218/.232 & .192/.23&.187/.24	 & .19/.23 &.168/.23	 &.168/.241	 &.19/.241   \\
 %\bf    GR  $\boldsymbol{\bar{\mathcal{L}}_S}$ 	    &  .089/.098 & .075/.097&.072/.105	 & .074/.097 &.06/.097	 &.06/.105	 &.075/.105   \\
 \hline 
 \bf GR\textsubscript{H}$\boldsymbol{\bar{\mathcal{E}}_S}$ 		&  .21/.215  & .18/.211	&.169/.228	 & .172/.207 &.127/.206	 &.133/.229	 &.179/.232   \\
% \bf   GR\textsubscript{H}  $\boldsymbol{\bar{\mathcal{R}}_S}$ 	&  .085/.087 & .067/.084&.063/.097   & .064/.082 &.038/.081  &.04/.096	 &.067/.099   \\
 \hline  
 \bf GP   $\boldsymbol{\bar{\mathcal{E}}_S}$ &\multicolumn{7}{|c|}{.126/.204}  \\
% \bf 	GP  $\boldsymbol{\bar{\mathcal{R}}_S}$ &\multicolumn{7}{|c|}{.037/.08}  \\
  \hline 
   \bf GP\textsubscript{App} $\boldsymbol{\bar{\mathcal{E}}_S}$ &\multicolumn{7}{|c|}{.159/.225}  \\
%   \bf GP\textsubscript{App}	   $\boldsymbol{\bar{\mathcal{R}}_S}$ &\multicolumn{7}{|c|}{.052/.089}  \\
  \hline 
 \end{tabular}
 \vspace{-1mm}
  \caption{Sequential BA $\nu =1.9$: Performance of the learning over the stochastic data under different feature availability. Note that on average $48.4$\% of the labels are $"1"$.}
   \vspace{-5mm}
 \label{Tab:ResultsSeqNu1.9}
\end{table*}
 

==> VAWorkedOutExample.tex <==
\subsection{A Worked-out VA Labeling Example}
 
 In the following example, we use the first five time steps of one of the sequences in the ray-tracing dataset. In chosen sequence, no outage or change in the best beam combination occur (for clarity of the presentation). The possible transferred data in one time-step and the and total received data up to that state are shown the table below. Note here we use the data transfer (i.e., multiply (\ref{eq:ratediscount}) by $T_f$, where we here used $T_f = 2.6$s). We use the table instead of trellis for clarity.
\begin{figure*}[!htb]
\vspace{-20mm}
 \scriptsize

\centering
\vspace{-4mm}

\includegraphics[width=1\columnwidth, trim={0.0cm 0cm 0cm 0cm},clip]{TheVATable2.pdf}
\vspace{-35mm}
\caption{An example of labeling a sequence of length five time-frames. Two states in each band. Although we display all the transitions from previous states to the next states (i.e., from any of the four previous states), due to the need for major beam search, some of these transitions are not possible and are thus marked by 'X'. In each entry, we show the transferred data (after discounting the time needed for beam-search) in that state and the accumulated data up to that state, respectively, separated by "/". The selected route in a given state is underlined. The final route is marked with bold font.}
\label{Fig:Nu19CirclevsQ}
 \vspace{-6mm}

\end{figure*}

%In the subsequent description, we use the words "cmWave major" for the best state that can be found based on a major beamsearch in the cm-wave band (for a definition of a "major beamsearch", please see the paper). The word "cmWave minor" refers to the best state that can be found from a minor beamsearch (whose results are predicated on the latest major beamsearch before that). The words "mmWave major" and "mmWave minor" are used completely analogously. 
At T=1, we assume that a major search has to be done in both cmWave and mmWave. The accumulated data will be just the possible transferred data in each state (after the major search). In both cases, the best beam combination should be discovered. Next, the mmWave major and cmWave major become the previous state for the next four states. In the next step, we can now do a cmWave minor search (which can only be reached through the cmWave major search in the previous step); the used beam in this case is the best beam in the current candidate list (discovered from the previous major search in cmWave), in the current example this is the best beam combination. As reminder, by definition of the protocol, a cmWave major search cannot be followed by another cmWave major search (unless there is an outage or in periodic major beam search). The accumulated data is the transferred data in the current band (after a minor search) added to the accumulated data from the previous state in cmWave major. The other state in this time step (T=2) is the cmWave major, and this could be reached only if there is an outage in power in cmWave or if the previous state is in the mmWave band (i.e., after band switching). For this time instant (T=2), it is only coming from mmWave major. The accumulated data in this case will be the data in mmWave at T =1 and the possible data transfer (after a major search) in cmWave at T=2. The same procedure follows for the mmWave states in this time step.
We elaborate in the next time step, T=3, where the current states are:
\begin{itemize}
\item cmWave minor, with previous states: cmWave minor (with accumulated data 34.96MB), and cmWave major (with accumulated data 19.9MB), for both the best beam in this time step is in the current candidate set, i.e., both can transfer 20.71MB with only minor search. Between the two, the selected route is underlined with a total data transfer of 55.68MB (from the previous cmWave minor). Note that in this case the current candidate list is same as the candidate list of previous cmWave minor.
    \item cmWave major, previous state: mmWave minor (with accumulated data of 10.27MB) and mmWave major (with accumulated data of 18.77MB). Note here we do not have a transition from cmWave minor as no outage is detected with a minor search (details are skipped), thus only the two possible states are from the mmWave. For both of them the possible data transfer (after major search) is, 18.46MB. Then the accumulated data will be larger for the route from mmWave major, with 37.23MB.
    \item mmWave minor, previous state: mmWave minor (with accumulated rate 10.27MB) and mmWave major (with accumulated rate 18.77MB). Similar to the cmWave minor, this state is accessible from the in-band transition, i.e., mmWave minor and major for this state. Luckily for this example, the current best beam combination is in the two previous candidate lists, so for both we can achieve a transferred data of 62.92MB with a minor search. Adding this value to the above we see that the rate obtained by a trajectory from mmWave major is higher and thus it is selected. The accumulated data is now  81.68MB
    \item mmWave major, previous state:cmWave minor (with accumulated data of 34.96MB) and cmWave major (with accumulated data of 19.9MB). The concept for this is similar to the cmWave major. For both previous states we will achieve a total data transfer of 34.25MB. However, the accumulated data from the cmWave minor is higher and thus that route is selected, resulting in accumulated data of of 69.21MB.
\end{itemize}
 
For the next time-frame, T=4, the process is the same for cmWave major and minor, however, for the mmWave a major search is enforced due to the periodic major search after 4 time frames. Which results in four possible previous states to the mmWave major and no transitions to the mmWave minor state.

For the last time frame, T=5, we see that the mmWave minor as a previous state is missing due to the description above. After going through the possible transitions, we see that the highest accumulated possible data transfer is highlighted in red in the table with mmWave minor state, preceded by mmWave major state. Tracking back the states, we have the following:
cmWave major$\longrightarrow$ cmWave Major $\longrightarrow$ mmWave minor $\longrightarrow$ mmWave Major $\longrightarrow$mmWave minor, the labeled sequence is [0 1 1 1 1]. With a total data transfer of 177.6MB, which is equal to the optimal value (based on a brute-force search). Now applying the same rules above to the [0 0 1 1 1] sequence (e.g., enforcing the mmWave major search in time step 4 and carrying on the candidate lists) the total rate is 165.17MB.

